TimeSeriesBench: An Industrial-Grade Benchmark for Time Series Anomaly Detection Models

Time series anomaly detection (TSAD) has gained significant attention due to its real-world applications to improve the stability of modern software systems. However, there is no effective way to verify whether they can meet the requirements for real-world deployment. Firstly, current algorithms typically train a specific model for each time series. Maintaining such many models is impractical in a large-scale system with tens of thousands of curves. The performance of using merely one unified model to detect anomalies remains unknown. Secondly, most TSAD models are trained on the historical part of a time series and are tested on its future segment. In distributed systems, however, there are frequent system deployments and upgrades, with new, previously unseen time series emerging daily. The performance of testing newly incoming unseen time series on current TSAD algorithms remains unknown. Lastly, the assumptions of the evaluation metrics in existing benchmarks are far from practical demands. To solve the above-mentioned problems, we propose an industrial-grade benchmark TimeSeriesBench. We assess the performance of existing algorithms across more than 168 evaluation settings and provide comprehensive analysis for the future design of anomaly detection algorithms. An industrial dataset is also released along with TimeSeriesBench.

==> tables/diff.tex <==
\begin{table*}[t]
    \centering
    \caption{The effect of whether employing first-order difference or not under all-in-one learning schema and reduced-length $F1_{best}$ metric. Best scores are highlighted in bold, and second-best scores are highlighted in bold and underlined. Performance improvements exceeding 5\% are marked with {\color{blue} $\uparrow$}, while performance declines exceeding 5\% are marked with {\color{red} $\downarrow$}.}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{c|cc|cc|cc|cc|cc|cc}
    \hline
        \multirow{2}{*}{\textbf{Method}}  & \multicolumn{2}{c|}{KPI}   & \multicolumn{2}{c|}{NAB} & \multicolumn{2}{c|}{TODS} & \multicolumn{2}{c|}{WSD}  & \multicolumn{2}{c|}{Yahoo} & \multicolumn{2}{c}{UCR}\\
        & $raw$ & $diff_1$ & $raw$ & $diff_1$ & $raw$ & $diff_1$ & $raw$ & $diff_1$ & $raw$ & $diff_1$ & $raw$ & $diff_1$  \\ \hline

        AR & \textbf{0.8179} & \underline{\textbf{0.8317}} & \textbf{0.9023} & \textbf{0.88} & 0.7624 & 0.7559 & 0.9381 & \textbf{0.9271} & \underline{\textbf{0.9301}} & \textbf{0.9484} & 0.4196 & 0.4328 \\
        LSTMAD-$\alpha$ & \underline{\textbf{0.8141}} & \textbf{0.8335} & 0.8468 & 0.8626 & 0.7402 & \underline{\textbf{0.9397}} {\color{blue} $\uparrow$} & \underline{\textbf{0.9481}} & \underline{\textbf{0.9166}} & 0.8101 & 0.9377  {\color{blue} $\uparrow$} & \textbf{0.5734} & \textbf{0.5868} \\ 
        LSTMAD-$\beta$ & 0.8135 & 0.8308 & 0.8484 & \underline{\textbf{0.8773}} & \underline{\textbf{0.7704}} & 0.9366 {\color{blue} $\uparrow$} & \textbf{0.9484} & 0.9117 & 0.767 & 0.9358 {\color{blue} $\uparrow$}  & \underline{\textbf{0.5476}} & \underline{\textbf{0.541}} \\ 
        AE & 0.7486 & 0.8173 {\color{blue} $\uparrow$}  & 0.8264 & 0.8578 & 0.728 & \textbf{0.9411} {\color{blue} $\uparrow$}  & 0.9174 & 0.9006 & 0.8144 & 0.9371 {\color{blue} $\uparrow$}  & 0.3537 & 0.4364 {\color{blue} $\uparrow$}  \\ 
        EncDecAD & 0.7317 & 0.731 & \underline{\textbf{0.8567}} & 0.8697 & 0.7274 & 0.8668 {\color{blue} $\uparrow$}  & 0.8254 & 0.8674 {\color{blue} $\uparrow$}  & 0.581 & 0.9108 {\color{blue} $\uparrow$}  & 0.35 & 0.4776 {\color{blue} $\uparrow$} \\ 
        SRCNN & 0.6363 & 0.6738 {\color{blue} $\uparrow$} & 0.6948 & 0.7698 {\color{blue} $\uparrow$}  & 0.3126 & 0.3727 {\color{blue} $\uparrow$}  & 0.7656 & 0.7794 & 0.6162 & 0.6702 {\color{blue} $\uparrow$}  & 0.2637 & 0.3712 {\color{blue} $\uparrow$}  \\ 
        AnomalyTransformer & 0.4693 & 0.697 {\color{blue} $\uparrow$}  & 0.7956 & 0.5533 {\color{red} $\downarrow$}  & 0.2444 & 0.4677 {\color{blue} $\uparrow$}  & 0.5865 & 0.6425 {\color{blue} $\uparrow$}  & 0.2907 & 0.6648 {\color{blue} $\uparrow$}  & 0.2209 & 0.4052 {\color{blue} $\uparrow$}  \\ 
        TimesNet & 0.4151 & 0.5762 {\color{blue} $\uparrow$}  & 0.839 & 0.8616 & 0.5219 & 0.8122 {\color{blue} $\uparrow$}  & 0.6953 & 0.7473 {\color{blue} $\uparrow$}  & 0.8435 & 0.9403 {\color{blue} $\uparrow$}  & 0.2904 & 0.3824 {\color{blue} $\uparrow$}  \\ 
        Donut & 0.6362 & 0.7262 {\color{blue} $\uparrow$}  & 0.7476 & 0.753 & \textbf{0.8721} & 0.8853 & 0.8154 & 0.8367 & 0.6323 & \underline{\textbf{0.9467}} {\color{blue} $\uparrow$}  & 0.322 & 0.5156 {\color{blue} $\uparrow$}  \\ 
        TFAD & 0.4198 & 0.373 {\color{red} $\downarrow$}  & 0.6948 & 0.1601 {\color{red} $\downarrow$}  & 0.5425 & 0.4494 {\color{red} $\downarrow$}  & 0.3235 & 0.2811 {\color{red} $\downarrow$}  & \textbf{0.9351} & 0.9287 & 0.4395 & 0.3788 {\color{red} $\downarrow$}  \\ \hline
        
    \end{tabular}
    }
    \label{tb:diff}
\end{table*}

==> tables/main_aio.tex <==
\begin{table*}[htb]
    \centering
    \caption{Performance comparison using all-in-one learning schema under reduced-length $F1_{best}$ and $AUPRC$.}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{c|cc|cc|cc|cc|cc|cc|cc}
    \hline
        \multirow{2}{*}{\textbf{Method}} & \multicolumn{2}{c|}{AIOPS} & \multicolumn{2}{c|}{NAB} & \multicolumn{2}{c|}{TODS} & \multicolumn{2}{c|}{WSD} & \multicolumn{2}{c|}{Yahoo} & \multicolumn{2}{c|}{UCR} & \multicolumn{2}{c}{NEK} \\
         & $F1_{best}$ & $AUPRC$ & $F1_{best}$ & $AUPRC$ & $F1_{best}$ & $AUPRC$ & $F1_{best}$ & $AUPRC$ & $F1_{best}$ & $AUPRC$ & $F1_{best}$ & $AUPRC$ & $F1_{best}$ & $AUPRC$ \\
    \hline
        MatrixProfile & - & - & - & - & - & - & - & - & - & - & - & - & - & -  \\
        SAND & - & - & - & - & - & - & - & - & - & - & - & - & - & -  \\
        Sub-LOF & - & - & - & - & - & - & - & - & - & - & - & - & - & -  \\
        AR & \textbf{0.8214} & 0.8203 & \textbf{0.8881} & \textbf{\underline{0.8462}} & 0.7859 & 0.8365 & 0.9276 & 0.9179 & \textbf{0.948} & \textbf{0.9392} & 0.4636 & 0.4182 & \textbf{\underline{0.9612}} & 0.9719 \\
        LSTMAD-$\alpha$ & 0.8141 & \textbf{\underline{0.8343}} & 0.8492 & 0.7889 & 0.7538 & 0.7738 & \textbf{0.9467} & \textbf{0.9401} & 0.8 & 0.7829 & \textbf{0.6144} & \textbf{\underline{0.5598}} & 0.9349 & 0.9528 \\
        LSTMAD-$\beta$ & \textbf{\underline{0.8151}} & \textbf{0.8377} & 0.8484 & 0.7821 & 0.7495 & 0.7771 & \textbf{\underline{0.9445}} & \textbf{\underline{0.9391}} & 0.8114 & 0.7922 & \textbf{\underline{0.6101}} & \textbf{0.5602} & 0.961 & \textbf{0.9781} \\
        AE & 0.7448 & 0.7523 & 0.8375 & 0.7793 & 0.7712 & 0.7441 & 0.9192 & 0.9138 & 0.8205 & 0.8018 & 0.3644 & 0.3208 & 0.9609 & \textbf{\underline{0.9757}} \\
        EncDecAD & 0.7003 & 0.6894 & 0.8336 & 0.7786 & 0.6534 & 0.6592 & 0.8353 & 0.8182 & 0.5842 & 0.5378 & 0.3333 & 0.2867 & 0.9534 & 0.9538 \\
        Donut & 0.5827 & 0.5578 & 0.7966 & 0.7085 & \textbf{\underline{0.836}} & \textbf{\underline{0.8381}} & 0.7666 & 0.7271 & 0.6498 & 0.6161 & 0.4 & 0.3395 & 0.5801 & 0.4923 \\
        FCVAE & 0.7593 & 0.7521 & \textbf{\underline{0.8857}} & \textbf{0.8587} & \textbf{0.8526} & \textbf{0.8535} & 0.8121 & 0.7814 & 0.8537 & 0.8292 & 0.4766 & 0.418 & 0.8148 & 0.793 \\
        SRCNN & 0.6672 & 0.632 & 0.635 & 0.5648 & 0.2598 & 0.1658 & 0.7742 & 0.7337 & 0.1728 & 0.1056 & 0.3791 & 0.3176 & 0.6173 & 0.5906 \\
        AnomalyTransformer & 0.3656 & 0.2103 & 0.7322 & 0.6432 & 0.2631 & 0.1561 & 0.5838 & 0.4227 & 0.2377 & 0.1468 & 0.2372 & 0.1777 & 0.666 & 0.5539 \\
        TFAD & 0.4889 & 0.4062 & 0.4679 & 0.3996 & 0.5626 & 0.5411 & 0.8016 & 0.7602 & \textbf{\underline{0.9361}} & \textbf{\underline{0.9236}} & 0.4941 & 0.4646 & 0.4103 & 0.2853 \\
        TranAD & 0.6561 & 0.6049 & 0.8567 & 0.7921 & 0.5624 & 0.5291 & 0.7409 & 0.6995 & 0.5211 & 0.4643 & 0.2483 & 0.2181 & 0.9571 & 0.9524 \\
        TimesNet & 0.4988 & 0.4657 & 0.8544 & 0.8055 & 0.5032 & 0.4293 & 0.539 & 0.4602 & 0.5341 & 0.5098 & 0.1856 & 0.149 & 0.9257 & 0.9459 \\
        OFA & 0.5544 & 0.4993 & 0.861 & 0.7911 & 0.6187 & 0.6129 & 0.8111 & 0.7877 & 0.766 & 0.7414 & 0.2888 & 0.2334 & 0.7642 & 0.7389 \\
        FITS & 0.6986 & 0.6966 & 0.8683 & 0.8196 & 0.7146 & 0.7446 & 0.8788 & 0.8745 & 0.9261 & 0.9189 & 0.428 & 0.391 & \textbf{0.9625} & 0.9719 \\
    \hline
    \end{tabular}
    }
    \label{tb:main_aio}
\end{table*}

==> tables/main_obo.tex <==

\begin{table*}[htb]
    \centering
    \caption{Performance comparison using naive learning schema under reduced-length $F1_{best}$ and $AUPRC$.}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{c|cc|cc|cc|cc|cc|cc|cc}
    \hline
        \multirow{2}{*}{\textbf{Method}} & 
        \multicolumn{2}{c|}{AIOPS} & \multicolumn{2}{c|}{NAB} & \multicolumn{2}{c|}{TODS} & \multicolumn{2}{c|}{WSD} & \multicolumn{2}{c|}{Yahoo} & \multicolumn{2}{c|}{UCR} & \multicolumn{2}{c}{NEK} \\
        & $F1_{best}$ & $AUPRC$ & $F1_{best}$ & $AUPRC$ & $F1_{best}$ & $AUPRC$ & $F1_{best}$ & $AUPRC$ & $F1_{best}$ & $AUPRC$ & $F1_{best}$ & $AUPRC$ & $F1_{best}$ & $AUPRC$ \\
    \hline
        MatrixProfile & 0.0281 & 0.0097 & 0.1769 & 0.0975 & 0.2058 & 0.1407 & 0.0371 & 0.0234 & 0.2051 & 0.1445 & 0.5066 & 0.4711 & 0.3163 & 0.2439 \\
        SAND & 0.0674 & 0.0262 & 0.3036 & 0.2169 & 0.2544 & 0.1879 & 0.0952 & 0.0666 & 0.468 & 0.4343 & 0.5494 & \textbf{\underline{0.5344}} & 0.1758 & 0.1304 \\
        Sub-LOF & 0.3764 & 0.31 & 0.6982 & 0.5835 & 0.5791 & 0.5236 & 0.7194 & 0.6895 & 0.4875 & 0.4443 & \textbf{\underline{0.5806}} & 0.5325 & 0.6807 & 0.6423 \\
        AR & 0.7517 & 0.75 & \textbf{\underline{0.9035}} & \textbf{0.8691} & \textbf{\underline{0.7472}} & \textbf{\underline{0.7677}} & 0.868 & 0.8609 & \textbf{0.9195} & \textbf{0.9057} & 0.4454 & 0.4026 & 
        0.9555 & 0.9647 \\
        LSTMAD-$\alpha$ & \textbf{0.8081} & \textbf{0.8236} & 0.8984 & 0.8358 & 0.7015 & 0.7201 & \textbf{\underline{0.9381}} & \textbf{\underline{0.9298}} & 0.5496 & 0.5026 & 0.4836 & 0.441 & \textbf{0.9971} & \textbf{0.9959} \\
        LSTMAD-$\beta$ & \textbf{\underline{0.8034}} & \textbf{\underline{0.8219}} & 0.9031 & 0.841 & \textbf{0.7589} & \textbf{0.7706} & \textbf{0.939} & \textbf{0.9309} & 0.5366 & 0.4868 & 0.4366 & 0.3931 & 0.9744 & 0.9716 \\
        AE & 0.7222 & 0.7295 & 0.8751 & 0.8146 & 0.6842 & 0.6675 & 0.918 & 0.9049 & 0.612 & 0.5692 & 0.4198 & 0.3879 & 0.9801 & 0.9824 \\
        EncDecAD & 0.7583 & 0.7621 & 0.8752 & 0.8136 & 0.6359 & 0.6234 & 0.9285 & 0.9214 & 0.5018 & 0.449 & 0.3178 & 0.2829 & 0.755 & 0.733 \\
        Donut & 0.6957 & 0.6791 & 0.8397 & 0.7607 & 0.7207 & 0.7061 & 0.8787 & 0.8668 & 0.6813 & 0.6441 & 0.4409 & 0.3968 & \textbf{\underline{0.9885}} & \textbf{\underline{0.9923}} \\
        FCVAE & 0.7851 & 0.8079 & 0.874 & 0.8539 & 0.7145 & 0.7162 & 0.9087 & 0.8966 & 0.6883 & 0.6498 & \textbf{0.5873} & \textbf{0.5482} & 0.8977 & 0.9128 \\
        SRCNN & 0.1627 & 0.0972 & 0.5802 & 0.4946 & 0.3042 & 0.1931 & 0.1785 & 0.0993 & 0.1261 & 0.0662 & 0.3227 & 0.2667 & 0.4365 & 0.3501 \\
        AnomalyTransformer & 0.3728 & 0.3053 & 0.7739 & 0.691 & 0.2827 & 0.182 & 0.2984 & 0.2128 & 0.145 & 0.0879 & 0.3104 & 0.2548 & 0.3997 & 0.2617 \\
        TFAD & 0.3551 & 0.2529 & 0.5746 & 0.532 & 0.4526 & 0.3943 & 0.7561 & 0.7115 & \textbf{\underline{0.781}} & \textbf{\underline{0.7501}} & 0.3398 & 0.3077 & 0.625 & 0.5786 \\
        TranAD & 0.6486 & 0.5798 & \textbf{0.9101} & \textbf{\underline{0.8627}} & 0.2531 & 0.1988 & 0.6738 & 0.6089 & 0.562 & 0.516 & 0.2527 & 0.2199 & 0.9071 & 0.8928 \\
        TimesNet & 0.6737 & 0.6674 & 0.8419 & 0.7845 & 0.3695 & 0.3327 & 0.8684 & 0.8466 & 0.4444 & 0.4089 & 0.2493 & 0.2142 & 0.9335 & 0.9388 \\
        OFA & 0.6891 & 0.6973 & 0.8869 & 0.8468 & 0.6263 & 0.5683 & 0.8784 & 0.8683 & 0.7512 & 0.7145 & 0.4169 & 0.3804 & 0.9471 & 0.9553 \\
        FITS & 0.7139 & 0.7187 & 0.8617 & 0.8168 & 0.5371 & 0.5119 & 0.8796 & 0.8822 & 0.7564 & 0.7235 & 0.4092 & 0.3657 & 0.8975 & 0.9032 \\
    \hline
    \end{tabular}
    }
    \label{tb:main_obo}
\end{table*}

==> tables/main_zeroshot.tex <==
\begin{table*}[htb]
    \centering
    \caption{Performance comparison using zero-shot learning schema under reduced-length $F1_{best}$ and $AUPRC$.}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{c|cc|cc|cc|cc|cc|cc|cc}
    \hline
        \multirow{2}{*}{\textbf{Method}} & \multicolumn{2}{c|}{AIOPS} & \multicolumn{2}{c|}{NAB} & \multicolumn{2}{c|}{TODS} & \multicolumn{2}{c|}{WSD} & \multicolumn{2}{c|}{Yahoo} & \multicolumn{2}{c|}{UCR} & \multicolumn{2}{c}{NEK} \\
         & $F1_{best}$ & $AUPRC$ & $F1_{best}$ & $AUPRC$ & $F1_{best}$ & $AUPRC$ & $F1_{best}$ & $AUPRC$ & $F1_{best}$ & $AUPRC$ & $F1_{best}$ & $AUPRC$ & $F1_{best}$ & $AUPRC$ \\
    \hline
        MatrixProfile & - & - & - & - & - & - & - & - & - & - & - & - & - & -  \\
        SAND & - & - & - & - & - & - & - & - & - & - & - & - & - & -  \\
        Sub-LOF & - & - & - & - & - & - & - & - & - & - & - & - & - & -  \\
        AR & 0.8013 & 0.7928 & 0.8967 & 0.8306 & \textbf{\underline{0.7975}} & \textbf{0.8589} & 0.926 & 0.9066 & \textbf{0.9366} & \textbf{\underline{0.9234}} & 0.487 & 0.443 & \textbf{0.9641} & \textbf{\underline{0.9723}} \\
        LSTMAD-$\alpha$ & \textbf{0.8184} & \textbf{0.8304} & 0.8593 & 0.7913 & 0.677 & 0.6834 & \textbf{\underline{0.9349}} & \textbf{\underline{0.92}} & 0.8277 & 0.8141 & \textbf{0.5927} & \textbf{0.539} & 0.9539 & 0.9692 \\
        LSTMAD-$\beta$ & \textbf{\underline{0.8073}} & \textbf{\underline{0.8233}} & 0.8556 & 0.7915 & 0.593 & 0.5935 & \textbf{0.9357} & \textbf{0.9219} & 0.7942 & 0.7745 & \textbf{\underline{0.5603}} & \textbf{\underline{0.5128}} & 0.9613 & 0.9718 \\
        AE & 0.7689 & 0.7787 & 0.8538 & 0.7917 & 0.7105 & 0.6926 & 0.8969 & 0.8841 & 0.8595 & 0.8437 & 0.3239 & 0.284 & 0.9591 & \textbf{0.9727} \\
        EncDecAD & 0.7537 & 0.7694 & 0.85 & 0.7796 & 0.7089 & 0.6829 & 0.8306 & 0.8163 & 0.5958 & 0.5499 & 0.3209 & 0.2764 & 0.9441 & 0.9526 \\
        Donut & 0.6863 & 0.6724 & 0.7187 & 0.603 & 0.6223 & 0.5933 & 0.7934 & 0.7568 & 0.7034 & 0.6733 & 0.4148 & 0.367 & 0.6204 & 0.5069 \\
        FCVAE & 0.7983 & 0.8143 & \textbf{0.9385} & \textbf{0.8895} & \textbf{0.7987} & \textbf{\underline{0.7884}} & 0.7707 & 0.7316 & 0.796 & 0.7683 & 0.4101 & 0.3642 & 0.7979 & 0.8044 \\
        SRCNN & 0.6888 & 0.6507 & 0.6421 & 0.6205 & 0.2977 & 0.18 & 0.7414 & 0.6936 & 0.1437 & 0.0859 & 0.3582 & 0.2889 & 0.5261 & 0.4788 \\
        AnomalyTransformer & 0.4361 & 0.2757 & 0.5601 & 0.4912 & 0.2199 & 0.1531 & 0.3027 & 0.2065 & 0.4302 & 0.3613 & 0.2749 & 0.2116 & 0.5376 & 0.4876 \\
        TFAD & 0.4659 & 0.3392 & 0.2806 & 0.2419 & 0.6352 & 0.619 & 0.8902 & 0.8634 & 0.9312 & 0.916 & 0.4689 & 0.44 & 0.4527 & 0.3534 \\
        TranAD & 0.4662 & 0.3843 & \textbf{\underline{0.9333}} & \textbf{\underline{0.8698}} & 0.4013 & 0.3717 & 0.62 & 0.5454 & 0.4878 & 0.4344 & 0.292 & 0.2571 & 0.8868 & 0.8766 \\
        TimesNet & 0.489 & 0.4613 & 0.8788 & 0.8248 & 0.5654 & 0.5223 & 0.6151 & 0.5569 & 0.4492 & 0.4091 & 0.2564 & 0.2204 & 0.7233 & 0.6843 \\
        OFA & 0.5476 & 0.5042 & 0.8462 & 0.7761 & 0.6503 & 0.6112 & 0.8484 & 0.8265 & 0.8294 & 0.8134 & 0.3499 & 0.2869 & 0.8236 & 0.8421 \\
        FITS & 0.6748 & 0.6674 & 0.8808 & 0.8092 & 0.659 & 0.715 & 0.8803 & 0.8794 & \textbf{\underline{0.9316}} & \textbf{0.9254} & 0.4164 & 0.3766 & \textbf{\underline{0.9639}} & 0.9672 \\
    \hline
    \end{tabular}
    }
    \label{tb:main_zs}
\end{table*}

==> tables/pa_aio.tex <==
\begin{table*}[htb]
    \centering
    \caption{Performance comparison under point-wise PA (Point Adjustment), reduced-length PA and event-wise PA when using all-in-one training schema.}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{c|ccc|ccc|ccc|ccc|ccc|ccc|ccc}
    \hline
        \multirow{2}{*}{\textbf{Method}} & \multicolumn{3}{c|}{AIOPS} & \multicolumn{3}{c|}{NAB} & \multicolumn{3}{c|}{TODS} & \multicolumn{3}{c|}{WSD} & \multicolumn{3}{c|}{Yahoo} & \multicolumn{3}{c|}{UCR} & \multicolumn{3}{c}{NEK} \\
         & $F1_p$ & $F1_r$ & $F1_e$ & $F1_p$ & $F1_r$ & $F1_e$ & $F1_p$ & $F1_r$ & $F1_e$ & $F1_p$ & $F1_r$ & $F1_e$ & $F1_p$ & $F1_r$ & $F1_e$ & $F1_p$ & $F1_r$ & $F1_e$ & $F1_p$ & $F1_r$ & $F1_e$ \\    \hline
        MatrixProfile & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\
        SAND & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & -  \\
        Sub-LOF & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & -  \\
        AR & 0.9141 & \textbf{0.8214} & \textbf{0.7838} & \textbf{0.9978} & \textbf{0.8881} & 0.7452 & 0.8696 & 0.7859 & 0.745 & 0.9863 & 0.9276 & 0.8883 & \textbf{\underline{0.964}} & \textbf{0.948} & \textbf{0.9414} & 0.7983 & 0.4636 & 0.3792 & \textbf{\underline{0.9897}} & \textbf{\underline{0.9612}} & 0.9395 \\
        LSTMAD-$\alpha$ & \textbf{0.924} & 0.8141 & \textbf{\underline{0.775}} & 0.9891 & 0.8492 & 0.7363 & 0.8712 & 0.7538 & 0.7247 & \textbf{\underline{0.9899}} & \textbf{0.9467} & \textbf{0.9119} & 0.8342 & 0.8 & 0.7861 & \textbf{0.8915} & \textbf{0.6144} & \textbf{\underline{0.5098}} & 0.9795 & 0.9349 & 0.9204 \\
        LSTMAD-$\beta$ & \textbf{\underline{0.9235}} & \textbf{\underline{0.8151}} & 0.7744 & 0.989 & 0.8484 & 0.7367 & 0.8771 & 0.7495 & 0.7121 & \textbf{0.99} & \textbf{\underline{0.9445}} & \textbf{\underline{0.9091}} & 0.8455 & 0.8114 & 0.7953 & \textbf{\underline{0.8691}} & \textbf{\underline{0.6101}} & \textbf{0.5113} & \textbf{0.9906} & 0.961 & 0.9451 \\
        AE & 0.8994 & 0.7448 & 0.6908 & 0.9838 & 0.8375 & 0.7336 & \textbf{\underline{0.8997}} & 0.7712 & 0.7129 & 0.9844 & 0.9192 & 0.8835 & 0.8551 & 0.8205 & 0.805 & 0.7053 & 0.3644 & 0.2848 & 0.9892 & 0.9609 & \textbf{\underline{0.9489}} \\
        EncDecAD & 0.8527 & 0.7003 & 0.6405 & 0.9866 & 0.8336 & 0.7321 & 0.8367 & 0.6534 & 0.596 & 0.9274 & 0.8353 & 0.7969 & 0.6486 & 0.5842 & 0.5581 & 0.7167 & 0.3333 & 0.2486 & 0.9878 & 0.9534 & 0.9305 \\ 
        Donut & 0.818 & 0.5827 & 0.5197 & 0.988 & 0.7966 & 0.5949 & \textbf{0.9006} & \textbf{\underline{0.836}} & \textbf{\underline{0.8111}} & 0.9196 & 0.7666 & 0.7004 & 0.7144 & 0.6498 & 0.6209 & 0.7711 & 
        0.4 & 0.2896 & 0.8915 & 0.5801 & 0.4765 \\
        FCVAE & 0.8831 & 0.7593 & 0.7066 & 0.9962 & \textbf{\underline{0.8857}} & \textbf{0.7824} & 0.8989 & \textbf{0.8526} & \textbf{0.8321} & 0.9382 & 0.8121 & 0.7558 & 0.8782 & 0.8537 & 0.8408 & 0.8339 & 
        0.4766 & 0.3665 & 0.9613 & 0.8148 & 0.7436 \\
        SRCNN & 0.8444 & 0.6672 & 0.6023 & 0.9041 & 0.635 & 0.5129 & 0.5706 & 0.2598 & 0.1749 & 0.8906 & 0.7742 & 0.7165 & 0.2591 & 0.1728 & 0.1361 & 0.813 & 0.3791 & 0.2668 & 0.7491 & 0.6173 & 0.5637 \\     
        AnomalyTransformer & 0.5024 & 0.3656 & 0.2962 & 0.9784 & 0.7322 & 0.5551 & 0.5168 & 0.2631 & 0.1969 & 0.7379 & 0.5838 & 0.494 & 0.328 & 0.2377 & 0.1939 & 0.6563 & 0.2372 & 0.1443 & 0.8599 & 0.666 & 0.5899 \\
        TFAD & 0.7809 & 0.4889 & 0.3698 & 0.8816 & 0.4679 & 0.3274 & 0.7778 & 0.5626 & 0.4776 & 0.9436 & 0.8016 & 0.7128 & \textbf{0.9656} & \textbf{\underline{0.9361}} & 0.9176 & 0.7612 & 0.4941 & 0.439 & 0.8196 & 0.4103 & 0.2529 \\
        TranAD & 0.7401 & 0.6561 & 0.614 & \textbf{\underline{0.9965}} & 0.8567 & 0.7032 & 0.7134 & 0.5624 & 0.5413 & 0.8373 & 0.7409 & 0.702 & 0.582 & 0.5211 & 0.4978 & 0.6075 & 0.2483 & 0.1949 & 0.971 & 0.9571 & \textbf{0.9546} \\
        TimesNet & 0.7452 & 0.4988 & 0.4227 & 0.9879 & 0.8544 & 0.7505 & 0.7245 & 0.5032 & 0.424 & 0.7342 & 0.539 & 0.4556 & 0.5644 & 0.5341 & 0.5185 & 0.547 & 0.1856 & 0.1185 & 0.9796 & 0.9257 & 0.8947 \\   
        OFA & 0.7934 & 0.5544 & 0.4651 & 0.9879 & 0.861 & 0.7053 & 0.745 & 0.6187 & 0.5494 & 0.926 & 0.8111 & 0.7568 & 0.8251 & 0.766 & 0.7367 & 0.7415 & 0.2888 & 0.1914 & 0.9429 & 0.7642 & 0.6954 \\
        FITS & 0.8807 & 0.6986 & 0.623 & 0.9964 & 0.8683 & \textbf{\underline{0.7508}} & 0.8831 & 0.7146 & 0.6548 & 0.9684 & 0.8788 & 0.8315 & 0.9435 & 0.9261 & \textbf{\underline{0.9184}} & 0.7477 & 0.428 & 0.3584 & 0.9895 & \textbf{0.9625} & 0.9447 \\
    \hline
    \end{tabular}
    }
    \label{tb:pa_aio}
\end{table*}

==> tables/pa_obo.tex <==
\begin{table*}[htb]
    \centering
    \caption{Performance comparison under point-wise PA (Point Adjustment), reduced-length PA and event-wise PA when using naive training schema.}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{c|ccc|ccc|ccc|ccc|ccc|ccc|ccc}
    \hline
        \multirow{2}{*}{\textbf{Method}} & \multicolumn{3}{c|}{AIOPS} & \multicolumn{3}{c|}{NAB} & \multicolumn{3}{c|}{TODS} & \multicolumn{3}{c|}{WSD} & \multicolumn{3}{c|}{Yahoo} & \multicolumn{3}{c|}{UCR} & \multicolumn{3}{c}{NEK} \\
         & $F1_p$ & $F1_r$ & $F1_e$ & $F1_p$ & $F1_r$ & $F1_e$ & $F1_p$ & $F1_r$ & $F1_e$ & $F1_p$ & $F1_r$ & $F1_e$ & $F1_p$ & $F1_r$ & $F1_e$ & $F1_p$ & $F1_r$ & $F1_e$ & $F1_p$ & $F1_r$ & $F1_e$ \\
    \hline
        MatrixProfile & 0.1915 & 0.0281 & 0.0171 & 0.7873 & 0.1769 & 0.0567 & 0.5284 & 0.2058 & 0.1389 & 0.1233 & 0.0371 & 0.0279 & 0.3079 & 0.2051 & 0.1678 & 0.7992 & 0.5066 & 0.4438 & 0.6859 & 0.3163 & 0.232 \\
        SAND & 0.271 & 0.0674 & 0.0397 & 0.7007 & 0.3036 & 0.1179 & 0.5372 & 0.2544 & 0.1879 & 0.1761 & 0.0952 & 0.0839 & 0.5718 & 0.468 & 0.4235 & 0.7489 & 0.5494 & \textbf{0.525} & 0.5641 & 0.1758 & 0.1106 
        \\
        Sub-LOF & 0.7273 & 0.3764 & 0.2805 & 0.9787 & 0.6982 & 0.6221 & 0.7997 & 0.5791 & 0.4795 & 0.8683 & 0.7194 & 0.6585 & 0.572 & 0.4875 & 0.4453 & \textbf{0.8811} & \textbf{\underline{0.5806}} & 0.4917 & 
        0.884 & 0.6807 & 0.6171 \\
        AR & 0.8775 & 0.7517 & 0.6944 & \textbf{0.9982} & \textbf{\underline{0.9035}} & 0.78 & 0.8312 & \textbf{\underline{0.7472}} & \textbf{\underline{0.6987}} & 0.9624 & 0.868 & 0.8225 & \textbf{0.9448} & 
        \textbf{0.9195} & \textbf{0.9026} & 0.7897 & 0.4454 & 0.3693 & 0.9887 & 0.9555 & 0.9249 \\
        LSTMAD-$\alpha$ & \textbf{0.9296} & \textbf{0.8081} & \textbf{0.7671} & 0.9912 & 0.8984 & 0.7852 & 0.8226 & 0.7015 & 0.6582 & \textbf{0.9871} & \textbf{\underline{0.9381}} & \textbf{\underline{0.9009}} & 
        0.6137 & 0.5496 & 0.5244 & 0.7894 & 0.4836 & 0.4043 & \textbf{0.999} & \textbf{0.9971} & \textbf{0.9964} \\
        LSTMAD-$\beta$ & \textbf{\underline{0.9288}} & \textbf{\underline{0.8034}} & \textbf{\underline{0.763}} & 0.9906 & 0.9031 & 0.79 & \textbf{0.8724} & \textbf{0.7589} & \textbf{0.7206} & \textbf{\underline{0.9861}} & \textbf{0.939} & \textbf{0.9021} & 0.6013 & 0.5366 & 0.5102 & 0.7713 & 0.4366 & 0.3562 & 0.9865 & 0.9744 & 0.9692 \\
        AE & 0.8778 & 0.7222 & 0.6743 & 0.9921 & 0.8751 & 0.7738 & 0.8402 & 0.6842 & 0.6404 & 0.9809 & 0.918 & 0.8851 & 0.67 & 0.612 & 0.5891 & 0.7074 & 0.4198 & 0.3606 & 0.9938 & 0.9801 & 0.9698 \\
        EncDecAD & 0.9015 & 0.7583 & 0.7022 & 0.99 & 0.8752 & 0.77 & 0.7346 & 0.6359 & 0.6156 & 0.9826 & 0.9285 & 0.8945 & 0.5682 & 0.5018 & 0.4767 & 0.6685 & 0.3178 & 0.2541 & 0.9085 & 0.755 & 0.7015 \\     
        Donut & 0.8595 & 0.6957 & 0.6299 & 0.9834 & 0.8397 & 0.6938 & 0.8655 & 0.7207 & 0.6826 & 0.9637 & 0.8787 & 0.8326 & 0.7306 & 0.6813 & 0.6598 & 0.7514 & 0.4409 & 0.358 & \textbf{\underline{0.9968}} & \textbf{\underline{0.9885}} & \textbf{\underline{0.9879}} \\
        FCVAE & 0.9183 & 0.7851 & 0.7364 & 0.9948 & 0.874 & \textbf{\underline{0.7933}} & \textbf{\underline{0.8658}} & 0.7145 & 0.6689 & 0.9689 & 0.9087 & 0.8695 & 0.7334 & 0.6883 & 0.6699 & \textbf{\underline{0.8357}} & \textbf{0.5873} & \textbf{\underline{0.5126}} & 0.9733 & 0.8977 & 0.8733 \\
        SRCNN & 0.4069 & 0.1627 & 0.1338 & 0.9079 & 0.5802 & 0.4275 & 0.6298 & 0.3042 & 0.2066 & 0.401 & 0.1785 & 0.1221 & 0.2299 & 0.1261 & 0.0849 & 0.7496 & 0.3227 & 0.2209 & 0.778 & 0.4365 & 0.3082 \\     
        AnomalyTransformer & 0.6235 & 0.3728 & 0.3124 & 0.9757 & 0.7739 & 0.6117 & 0.5249 & 0.2827 & 0.2123 & 0.4414 & 0.2984 & 0.2462 & 0.2156 & 0.145 & 0.1193 & 0.7251 & 0.3104 & 0.2076 & 0.683 & 0.3997 & 0.3086 \\
        TFAD & 0.602 & 0.3551 & 0.2638 & 0.8609 & 0.5746 & 0.4979 & 0.6686 & 0.4526 & 0.3751 & 0.8572 & 0.7561 & 0.7113 & \textbf{\underline{0.8277}} & \textbf{\underline{0.781}} & \textbf{\underline{0.7581}} & 0.6456 & 0.3398 & 0.2846 & 0.8653 & 0.625 & 0.5245 \\
        TranAD & 0.7696 & 0.6486 & 0.6051 & \textbf{\underline{0.9975}} & \textbf{0.9101} & \textbf{0.8133} & 0.5131 & 0.2531 & 0.2127 & 0.7616 & 0.6738 & 0.6468 & 0.6222 & 0.562 & 0.539 & 0.6101 & 0.2527 & 0.1946 & 0.9481 & 0.9071 & 0.8924 \\
        TimesNet & 0.8018 & 0.6737 & 0.6379 & 0.9875 & 0.8419 & 0.7488 & 0.6234 & 0.3695 & 0.3048 & 0.9354 & 0.8684 & 0.8358 & 0.487 & 0.4444 & 0.4279 & 0.621 & 0.2493 & 0.1873 & 0.9807 & 0.9335 & 0.9098 \\  
        OFA & 0.881 & 0.6891 & 0.615 & 0.9962 & 0.8869 & 0.7841 & 0.6928 & 0.6263 & 0.5811 & 0.9564 & 0.8784 & 0.8344 & 0.7979 & 0.7512 & 0.7315 & 0.7286 & 0.4169 & 0.3489 & 0.9839 & 0.9471 & 0.927 \\        
        FITS & 0.9108 & 0.7139 & 0.6324 & 0.9962 & 0.8617 & 0.7447 & 0.7543 & 0.5371 & 0.4873 & 0.9705 & 0.8796 & 0.8377 & 0.8173 & 0.7564 & 0.7244 & 0.7567 & 0.4092 & 0.3284 & 0.9806 & 0.8975 & 0.8462 \\   
    \hline
    \end{tabular}
    }
    \label{tb:pa_obo}
\end{table*}

==> tables/pa_zs.tex <==
\begin{table*}[htb]
    \centering
    \caption{Performance comparison under point-wise PA (Point Adjustment), reduced-length PA and event-wise PA when using zero-shot learning schema.}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{c|ccc|ccc|ccc|ccc|ccc|ccc|ccc}
    \hline
        \multirow{2}{*}{\textbf{Method}} & \multicolumn{3}{c|}{AIOPS} & \multicolumn{3}{c|}{NAB} & \multicolumn{3}{c|}{TODS} & \multicolumn{3}{c|}{WSD} & \multicolumn{3}{c|}{Yahoo} & \multicolumn{3}{c|}{UCR} & \multicolumn{3}{c}{NEK} \\
         & $F1_p$ & $F1_r$ & $F1_e$ & $F1_p$ & $F1_r$ & $F1_e$ & $F1_p$ & $F1_r$ & $F1_e$ & $F1_p$ & $F1_r$ & $F1_e$ & $F1_p$ & $F1_r$ & $F1_e$ & $F1_p$ & $F1_r$ & $F1_e$ & $F1_p$ & $F1_r$ & $F1_e$ \\    
         \hline
        MatrixProfile & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\
        SAND & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & -  \\
        Sub-LOF & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & -  \\        
        AR & 0.8991 & 0.8013 & 0.7603 & 0.9981 & 0.8967 & 0.7467 & \textbf{0.9192} & \textbf{\underline{0.7975}} & \textbf{\underline{0.7697}} & 0.9886 & 0.926 & 0.8765 & \textbf{\underline{0.9535}} & \textbf{0.9366} & \textbf{0.9305} & 0.8221 & 0.487 & 0.4046 & 0.9893 & \textbf{0.9641} & 0.9371 \\
        LSTMAD-$\alpha$ & \textbf{0.9109} & \textbf{0.8184} & \textbf{0.7866} & 0.9966 & 0.8593 & 0.7127 & 0.8163 & 0.677 & 0.6485 & \textbf{0.9902} & \textbf{\underline{0.9349}} & \textbf{0.8899} & 0.86 & 0.8277 & 0.8147 & \textbf{0.8782} & \textbf{0.5927} & \textbf{0.4898} & 0.9879 & 0.9539 & \textbf{\underline{0.9478}} \\
        LSTMAD-$\beta$ & 0.9073 & \textbf{\underline{0.8073}} & \textbf{\underline{0.7763}} & 0.9967 & 0.8556 & 0.706 & 0.7793 & 0.593 & 0.5435 & \textbf{\underline{0.9892}} & \textbf{0.9357} & \textbf{\underline{0.8888}} & 0.8312 & 0.7942 & 0.7785 & \textbf{\underline{0.8367}} & \textbf{\underline{0.5603}} & \textbf{\underline{0.4681}} & 0.9878 & 0.9613 & \textbf{0.9573} \\
        AE & 0.8998 & 0.7689 & 0.7251 & 0.9961 & 0.8538 & 0.7133 & 0.8521 & 0.7105 & 0.6829 & 0.9787 & 0.8969 & 0.8603 & 0.8865 & 0.8595 & 0.8472 & 0.6793 & 0.3239 & 0.2497 & \textbf{0.9909} & 0.9591 & 0.9451 \\
        EncDecAD & 0.8873 & 0.7537 & 0.7097 & 0.9952 & 0.85 & 0.725 & 0.8139 & 0.7089 & 0.6862 & 0.9373 & 0.8306 & 0.7922 & 0.6596 & 0.5958 & 0.5668 & 0.7232 & 0.3209 & 0.243 & 0.986 & 0.9441 & 0.9332 \\     
        Donut & 0.8766 & 0.6863 & 0.6159 & 0.9928 & 0.7187 & 0.4022 & 0.8324 & 0.6223 & 0.5523 & 0.924 & 0.7934 & 0.722 & 0.7724 & 0.7034 & 0.6705 & 0.7511 & 0.4148 & 0.3297 & 0.9203 & 0.6204 & 0.5003 \\     
        FCVAE & \textbf{\underline{0.9096}} & 0.7983 & 0.7679 & \textbf{0.9991} & \textbf{0.9385} & \textbf{0.8133} & 0.8611 & \textbf{0.7987} & \textbf{0.7708} & 0.9145 & 0.7707 & 0.7184 & 0.8307 & 0.796 & 0.7778 & 0.7691 & 0.4101 & 0.325 & 0.9551 & 0.7979 & 0.7439 \\
        SRCNN & 0.8792 & 0.6888 & 0.626 & 0.9596 & 0.6421 & 0.6092 & 0.5896 & 0.2977 & 0.2307 & 0.8633 & 0.7414 & 0.6861 & 0.2384 & 0.1437 & 0.1051 & 0.8107 & 0.3582 & 0.2269 & 0.7105 & 0.5261 & 0.448 \\     
        AnomalyTransformer & 0.5934 & 0.4361 & 0.351 & 0.9526 & 0.5601 & 0.4222 & 0.388 & 0.2199 & 0.175 & 0.533 & 0.3027 & 0.2251 & 0.4807 & 0.4302 & 0.4069 & 0.7598 & 0.2749 & 0.1744 & 0.6492 & 0.5376 & 0.4969 \\
        TFAD & 0.805 & 0.4659 & 0.3241 & 0.9144 & 0.2806 & 0.2169 & 0.8302 & 0.6352 & 0.5554 & 0.9639 & 0.8902 & 0.833 & \textbf{0.9586} & 0.9312 & 0.9169 & 0.7316 & 0.4689 & 0.4156 & 0.8352 & 0.4527 & 0.3145 \\
        TranAD & 0.6288 & 0.4662 & 0.4031 & \textbf{\underline{0.9989}} & \textbf{\underline{0.9333}} & \textbf{\underline{0.8}} & 0.5918 & 0.4013 & 0.3485 & 0.7219 & 0.62 & 0.591 & 0.5579 & 0.4878 & 0.458 & 
        0.6554 & 0.292 & 0.2332 & 0.9258 & 0.8868 & 0.8842 \\
        TimesNet & 0.7622 & 0.489 & 0.4329 & 0.9974 & 0.8788 & 0.73 & 0.7976 & 0.5654 & 0.497 & 0.7777 & 0.6151 & 0.5544 & 0.5038 & 0.4492 & 0.4233 & 0.6406 & 0.2564 & 0.1945 & 0.9467 & 0.7233 & 0.5973 \\    
        OFA & 0.7912 & 0.5476 & 0.4538 & 0.9965 & 0.8462 & 0.6971 & 0.8413 & 0.6503 & 0.5877 & 0.9423 & 0.8484 & 0.8032 & 0.8749 & 0.8294 & 0.8083 & 0.7771 & 0.3499 & 0.2368 & 0.9497 & 0.8236 & 0.7615 \\     
        FITS & 0.8772 & 0.6748 & 0.586 & 0.9973 & 0.8808 & 0.7282 & \textbf{\underline{0.8688}} & 0.659 & 0.593 & 0.9678 & 0.8803 & 0.8406 & 0.9475 & \textbf{\underline{0.9316}} & \textbf{\underline{0.9233}} 
        & 0.7395 & 0.4164 & 0.339 & \textbf{\underline{0.9899}} & \textbf{\underline{0.9639}} & 0.9469 \\
    \hline
    \end{tabular}
    }
    \label{tb:pa_zs}
\end{table*}
